Ensemble-filtered vortex modeling of strongly disturbed aerodynamic flows

The task of dynamic flow estimation is to construct an approximation of an evolving flow---and particularly, its response to disturbances---using measurements from available sensors. Building from previous work by Darakananda et al.~(Phys Rev Fluids 2018), we further develop an ensemble Kalman filter (EnKF) framework for aerodynamic flows based on an ensemble of randomly-perturbed inviscid vortex models of flow about an infinitely-thin plate. In the forecast step, vortex elements in each ensemble member are advected by the flow and new elements are released from each edge of the plate; the elements are aggregated to maintain an efficient representation. The vortex elements and leading edge constraint are corrected in the analysis step by assimilating the surface pressure differences across the plate measured from the truth system. We show that the overall framework can be physically interpreted as a series of adjustments to the position and shape of an elliptical region of uncertainty associated with each vortex element. In this work, we compare the previously-used stochastic EnKF with the ensemble transform Kalman filter (ETKF), which uses a deterministic analysis step. We examine the response of the flat plate at $20^\circ$ in two perturbed flows, with truth data obtained from high-fidelity simulation at Reynolds number 500. In the first case, we apply a sequence of large-amplitude pulses near the leading edge of the plate to mimic flow actuation. In the second, we place the plate in a vortex street wake behind a cylinder. In both cases, we show that the vortex-based framework accurately estimates the pressure distribution and normal force, with no {\em a priori} knowledge of the perturbations. We show that the ETKF is consistently more robust than the stochastic EnKF. Finally, we examine the mapping from measurements to state update in the analysis step through SVD of the Kalman gain.

==> README <==

Here's a copy of my LaTeX2e style file for typesetting programs
and algorithms in my favourite style without having to type
in endless tabbing commands.  Each line is set in math mode
so all the indentation and spacing is done automatically.
The notation |variable_name| can be used within normal text,
maths expressions or programs to indicate a variable name.
Use \origbar to get a normal | symbol in a program.
The commands \A, \B, \R, \T and \Z typeset the corresponding bold
letter with the next object as a substript (eg \S1 typesets {\bf
S$_1$} etc). They now cope with primes as well, (eg $\S2'''$). The
program.sty file can be easily edited to reflect your favoured style.
Typesetting a program is as easy as:

\(\IF x \ne 0 \THEN |long_name|_{123} = x^y \FI\)

See the program-demo.tex file for examples.

The file should work with or without AMSLaTeX.

This work is released under the GPL version 3.

                        Martin Ward.

martin@gkc.org.uk  http://www.cse.dmu.ac.uk/~mward/  Erdos number: 4
G.K.Chesterton web site:  http://www.cse.dmu.ac.uk/~mward/gkc/


